Prompt Design Matters for Computational Social Science Tasks but in Unpredictable Ways

Manually annotating data for computational social science tasks can be costly, time-consuming, and emotionally draining. While recent work suggests that LLMs can perform such annotation tasks in zero-shot settings, little is known about how prompt design impacts LLMs' compliance and accuracy. We conduct a large-scale multi-prompt experiment to test how model selection (ChatGPT, PaLM2, and Falcon7b) and prompt design features (definition inclusion, output type, explanation, and prompt length) impact the compliance and accuracy of LLM-generated annotations on four CSS tasks (toxicity, sentiment, rumor stance, and news frames). Our results show that LLM compliance and accuracy are highly prompt-dependent. For instance, prompting for numerical scores instead of labels reduces all LLMs' compliance and accuracy. The overall best prompting setup is task-dependent, and minor prompt changes can cause large changes in the distribution of generated labels. By showing that prompt design significantly impacts the quality and distribution of LLM-generated annotations, this work serves as both a warning and practical guide for researchers and practitioners.

==> tables/OLD_STUFF/framing_sentiment.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{cl|ccc|ccc|ccc}
\multicolumn{1}{l}{}              &                                           & \multicolumn{3}{c|}{\textbf{Explanation}}                         & \multicolumn{3}{c|}{\textbf{Output type}}                              & \multicolumn{3}{c}{\textbf{Prompt length}}                                \\
\textbf{Model}                    & \multicolumn{1}{c|}{\textbf{Label class}} & \textbf{Yes} & \multicolumn{1}{c|}{\textbf{No}} & \textbf{$\Delta$}      & \textbf{Label} & \multicolumn{1}{c|}{\textbf{Score}} & \textbf{$\Delta$}      & \textbf{Standard} & \multicolumn{1}{c|}{\textbf{Concise}} & \textbf{$\Delta$}     \\ \hline
\multirow{5}{*}{\textbf{ChatGPT}} & very positive                             & 1.43         & \multicolumn{1}{c|}{5.05}        & -3.62           & 2.42           & \multicolumn{1}{c|}{4.1}            & -1.68           & 3.53              & \multicolumn{1}{c|}{2.97}             & 0.56           \\
                                  & somewhat positive                         & 16.74        & \multicolumn{1}{c|}{33.25}       & \textbf{-16.51} & 31.84          & \multicolumn{1}{c|}{18.17}          & \textbf{13.67}  & 19.96             & \multicolumn{1}{c|}{30.26}            & \textbf{-10.3} \\
                                  & neutral                                   & 54.37        & \multicolumn{1}{c|}{19.68}       & \textbf{34.69}  & 27.34          & \multicolumn{1}{c|}{46.58}          & \textbf{-19.24} & 39.02             & \multicolumn{1}{c|}{34.68}            & 4.34           \\
                                  & somewhat negative                         & 19.57        & \multicolumn{1}{c|}{26.12}       & -6.55  & 31.98          & \multicolumn{1}{c|}{13.59}          & \textbf{18.39}  & 20.94             & \multicolumn{1}{c|}{24.84}            & -3.9           \\
                                  & very negative                             & 7.89         & \multicolumn{1}{c|}{15.9}        & -8.01  & 6.41           & \multicolumn{1}{c|}{17.56}          & \textbf{-11.15} & 16.55             & \multicolumn{1}{c|}{7.24}             & 9.31  \\ \hline
\multirow{5}{*}{\textbf{PaLM2}}   & very positive                             & 22.53        & \multicolumn{1}{c|}{33.08}       & \textbf{-10.55} & 20.05          & \multicolumn{1}{c|}{33.47}          & \textbf{-13.42} & 26.11             & \multicolumn{1}{c|}{29.02}            & -2.91          \\
                                  & somewhat positive                         & 31.09        & \multicolumn{1}{c|}{25.15}       & 5.94   & 37.15          & \multicolumn{1}{c|}{21.05}          & \textbf{16.1}   & 28.48             & \multicolumn{1}{c|}{28.21}            & 0.27           \\
                                  & neutral                                   & 2.18         & \multicolumn{1}{c|}{2.08}        & 0.1             & 3.11           & \multicolumn{1}{c|}{1.32}           & 1.79            & 0.94              & \multicolumn{1}{c|}{3.69}             & -2.75          \\
                                  & somewhat negative                         & 26.47        & \multicolumn{1}{c|}{16.73}       & 9.74   & 25.91          & \multicolumn{1}{c|}{18.74}          & 7.17   & 24.15             & \multicolumn{1}{c|}{19.19}            & 4.96           \\
                                  & very negative                             & 17.72        & \multicolumn{1}{c|}{22.97}       & -5.25  & 13.78          & \multicolumn{1}{c|}{25.42}          & \textbf{-11.64} & 20.32             & \multicolumn{1}{c|}{19.89}            & 0.43          
\end{tabular}
}
\caption{Framing effect for sentiment: Differences in annotation class distribution due to different prompt designs. \sa{TBD highlight gains and losses in red/green}}
\label{tab:framing-sentiment}

\end{table*}

==> tables/OLD_STUFF/framing_stance.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\resizebox{\textwidth}{!}{
\begin{tabular}{cl|ccc|ccc|ccc|ccc}
\multicolumn{1}{l}{}              &                                           & \multicolumn{3}{c|}{\textbf{Definition}}                     & \multicolumn{3}{c|}{\textbf{Explanation}}                    & \multicolumn{3}{c|}{\textbf{Output type}}                         & \multicolumn{3}{c}{\textbf{Prompt length}}                             \\
\textbf{Model}                    & \multicolumn{1}{c|}{\textbf{Label class}} & \textbf{Yes} & \multicolumn{1}{c|}{\textbf{No}} & \textbf{$\Delta$} & \textbf{Yes} & \multicolumn{1}{c|}{\textbf{No}} & \textbf{$\Delta$} & \textbf{Label} & \multicolumn{1}{c|}{\textbf{Score}} & \textbf{$\Delta$} & \textbf{Standard} & \multicolumn{1}{c|}{\textbf{Concise}} & \textbf{$\Delta$} \\ \hline
\multirow{4}{*}{\textbf{ChatGPT}} & comment                                   & 63.64        & \multicolumn{1}{c|}{65.28}       & -1.64      & 67.2         & \multicolumn{1}{c|}{61.73}       & 5.47       & 74.38          & \multicolumn{1}{c|}{54.5}           & 19.88      & 66.85             & \multicolumn{1}{c|}{62.07}            & 4.78       \\
                                  & support                                   & 3.08         & \multicolumn{1}{c|}{3.44}        & -0.36      & 2.85         & \multicolumn{1}{c|}{3.67}        & -0.82      & 2.34           & \multicolumn{1}{c|}{4.19}           & -1.85      & 3.39              & \multicolumn{1}{c|}{3.13}             & 0.26       \\
                                  & deny                                      & 23.64        & \multicolumn{1}{c|}{25.97}       & -2.33      & 22.3         & \multicolumn{1}{c|}{27.3}        & -5         & 16.63          & \multicolumn{1}{c|}{33.01}          & -16.38     & 22.48             & \multicolumn{1}{c|}{27.14}            & -4.66      \\
                                  & question                                  & 9.64         & \multicolumn{1}{c|}{5.31}        & 4.33       & 7.64         & \multicolumn{1}{c|}{7.31}        & 0.33       & 6.65           & \multicolumn{1}{c|}{8.3}            & -1.65      & 7.29              & \multicolumn{1}{c|}{7.66}             & -0.37      \\ \hline
\multirow{4}{*}{\textbf{PaLM2}}   & comment                                   & 58.29        & \multicolumn{1}{c|}{61.52}       & -3.23      & 58.59        & \multicolumn{1}{c|}{61.43}       & -2.84      & 67.37          & \multicolumn{1}{c|}{50.31}          & 17.06      & 59.43             & \multicolumn{1}{c|}{60.44}            & -1.01      \\
                                  & deny                                      & 16.62        & \multicolumn{1}{c|}{16.94}       & -0.32      & 17.56        & \multicolumn{1}{c|}{16}          & 1.56       & 13.29          & \multicolumn{1}{c|}{21.39}          & -8.1       & 17.81             & \multicolumn{1}{c|}{16.01}            & 1.8        \\
                                  & support                                   & 19.53        & \multicolumn{1}{c|}{13.97}       & 5.56       & 18.19        & \multicolumn{1}{c|}{14.96}       & 3.23       & 13.33          & \multicolumn{1}{c|}{20.87}          & -7.54      & 15.09             & \multicolumn{1}{c|}{17.73}            & -2.64      \\
                                  & question                                  & 5.55         & \multicolumn{1}{c|}{7.57}        & -2.02      & 5.66         & \multicolumn{1}{c|}{7.6}         & -1.94      & 6.01           & \multicolumn{1}{c|}{7.43}           & -1.42      & 7.67              & \multicolumn{1}{c|}{5.82}             & 1.85      
\end{tabular}
}
\caption{Framing effect for rumor stance: Differences in annotation class distribution due to different prompt designs}
\label{tab:framing-stance}
\end{table*}

==> tables/OLD_STUFF/framing_toxicity.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\resizebox{\textwidth}{!}{

\begin{tabular}{cl|ccc|ccc|ccc|ccc}
\multicolumn{1}{l}{}              & \multicolumn{1}{l|}{} & \multicolumn{3}{c|}{\textbf{Definition}}                                                              & \multicolumn{3}{c|}{\textbf{Explanation}}                                                             & \multicolumn{3}{c|}{\textbf{Output type}}                                                                  & \multicolumn{3}{c}{\textbf{Prompt length}}                                                                     \\
\textbf{Model}                    & \textbf{Label class}  & \multicolumn{1}{c}{\textbf{Yes}} & \multicolumn{1}{c|}{\textbf{No}} & \multicolumn{1}{c|}{\textbf{$\Delta$}} & \multicolumn{1}{c}{\textbf{Yes}} & \multicolumn{1}{c|}{\textbf{No}} & \multicolumn{1}{c|}{\textbf{$\Delta$}} & \multicolumn{1}{c}{\textbf{Label}} & \multicolumn{1}{c|}{\textbf{Score}} & \multicolumn{1}{c|}{\textbf{$\Delta$}} & \multicolumn{1}{c}{\textbf{Standard}} & \multicolumn{1}{c|}{\textbf{Concise}} & \multicolumn{1}{c}{\textbf{$\Delta$}} \\
\hline
\multirow{2}{*}{\textbf{ChatGPT}} & True         & 39.69                            & \multicolumn{1}{l|}{43.07}       & -3.38                           & 41.15                            & \multicolumn{1}{l|}{41.61}       & -0.46                           & 38.15                              & \multicolumn{1}{l|}{44.62}          & -6.47                           & 38.84                                 & \multicolumn{1}{l|}{43.93}            & -5.09                          \\
                                  & False        & 60.31                            & \multicolumn{1}{l|}{56.93}       & 3.38                            & 58.85                            & \multicolumn{1}{l|}{58.39}       & 0.46                            & 61.85                              & \multicolumn{1}{l|}{55.38}          & 6.47                            & 61.16                                 & \multicolumn{1}{l|}{56.07}            & 5.09                           \\ \hline
\multirow{2}{*}{\textbf{PaLM2}}   & True         & 26.85                            & \multicolumn{1}{l|}{24.44}       & 2.41                            & 25.14                            & \multicolumn{1}{l|}{26.15}       & -1.01                           & 22.32                              & \multicolumn{1}{l|}{28.97}          & -6.65                           & 20.69                                 & \multicolumn{1}{l|}{30.60}            & -9.91                          \\
                                  & False        & 73.15                            & \multicolumn{1}{l|}{75.56}       & -2.41                           & 74.86                            & \multicolumn{1}{l|}{73.85}       & 1.01                            & 77.68                              & \multicolumn{1}{l|}{71.03}          & 6.65                            & 79.31                                 & \multicolumn{1}{l|}{69.40}            & 9.91                          
\end{tabular}
}
\caption{Framing effect for toxicity: Differences in annotation class distribution due to different prompt designs}
\label{tab:framing-toxicity}

\end{table*}

==> tables/OLD_STUFF/noncompliance_ex.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}

\begin{table*}[]
\begin{tabular}{@{}p{0.2\textwidth}p{0.2\textwidth}p{0.5\textwidth}p{0.1\textwidth}@{}}
\toprule
\multicolumn{2}{c}{\textbf{Experimental condition}}                                                                                                                                                     & \multicolumn{1}{c}{\textbf{LLM output}}                                                                                                                                                                                                                   & \multicolumn{1}{c}{\textbf{Cause of noncompliance}} \\ \midrule
\begin{tabular}[c]{@{}l@{}}Model: Falcon7b\\ Task: News frames\end{tabular}  & \begin{tabular}[c]{@{}l@{}}Definition: no\\ Explanation: no\\ Output type: score\\ Length: standard\end{tabular}  & Politics: 0.8, Public opinion: 0.8, Society and culture: 0.8, Economic consequences: 0.8, Gun rights: 0.8, Gun control: 0.8, Mental health: 0.8, School and public space safety: 0.8, Race and ethnicity: 0.8                                             & Unable to parse numerical scores                    \\
\begin{tabular}[c]{@{}l@{}}Model: Falcon7b\\ Task: Sentiment\end{tabular}    & \begin{tabular}[c]{@{}l@{}}Definition: no\\ Explanation: no\\ Output type: score\\ Length: standard\end{tabular}  & class1 0.8 class2 0.6 class3 0.4 class4 0.2 class5 0.8                                                                                                                                                                                                    & Incorrect class names                               \\
\begin{tabular}[c]{@{}l@{}}Model: Falcon7b\\ Task: Rumor stance\end{tabular} & \begin{tabular}[c]{@{}l@{}}Definition: no\\ Explanation: yes\\ Output type: score\\ Length: concise\end{tabular}  & Tweets 1 and 2 have opposing stances. The sentiment of Tweet 2 is more likely to be categorized as supporting, as it expresses agreement with the statement 'I'm with her scum.' The sum of the probability scores for these two tweets is 0.5 (denying). & Arbitrary output                                    \\
\begin{tabular}[c]{@{}l@{}}Model: Falcon7b\\ Task: Rumor stance\end{tabular} & \begin{tabular}[c]{@{}l@{}}Definition: yes\\ Explanation: no\\ Output type: label\\ Length: concise\end{tabular}  & Mike Pence is a hypocrite.                                                                                                                                                                                                                                & Arbitrary output                                    \\
\begin{tabular}[c]{@{}l@{}}Model: Falcon7b\\ Task: Toxicity\end{tabular}     & \begin{tabular}[c]{@{}l@{}}Definition: no\\ Explanation: no\\ Output type: label\\ Length: standard\end{tabular}  & trump2024, trump2020, trump2022, trump2021, trump2023, trump2025, trump2026, trump2027, trump2028....                                                                                                                                                     & Arbitrary output                                    \\
\begin{tabular}[c]{@{}l@{}}Model: PaLM2\\ Task: News frames\end{tabular}     & \begin{tabular}[c]{@{}l@{}}Definition: no\\ Explanation: no\\ Output type: label\\ Length: standard\end{tabular}  & I'm not able to help with that, as I'm only a language model. If you believe this is an error, please send us your feedback.                                                                                                                              & Refusal to generate output                          \\
\begin{tabular}[c]{@{}l@{}}Model: PaLM2\\ Task: Sentiment\end{tabular}       & \begin{tabular}[c]{@{}l@{}}Definition: no\\ Explanation: no\\ Output type: label\\ Length: concise\end{tabular}   & negative                                                                                                                                                                                                                                                  & Incorrect class names                               \\
\begin{tabular}[c]{@{}l@{}}Model: PaLM2\\ Task: Sentiment\end{tabular}       & \begin{tabular}[c]{@{}l@{}}Definition: no\\ Explanation: yes\\ Output type: label\\ Length: concise\end{tabular}  & Positive. The text is positive because it is praising the movie for its brave attempt to tap into the heartbeat of the world, its salute to the universal language of rhythm, and its zippy sampling of sounds.                                           & Incorrect class names                               \\
\begin{tabular}[c]{@{}l@{}}Model: PaLM2\\ Task: Rumor stance\end{tabular}    & \begin{tabular}[c]{@{}l@{}}Definition: yes\\ Explanation: no\\ Output type: score\\ Length: standard\end{tabular} & comment 0.0 0.0 0.0 1.0                                                                                                                                                                                                                                   & Unable to parse numerical scores                    \\
\begin{tabular}[c]{@{}l@{}}Model: ChatGPT\\ Task: Rumor stance\end{tabular}  & \begin{tabular}[c]{@{}l@{}}Definition: yes\\ Explanation: yes\\ Output type: score\\ Length: concise\end{tabular} & \begin{tabular}[c]{@{}l@{}}Tweet 2's stance towards Tweet 1:\\ - Support: 0\%\\ - Deny: 0\%\\ - Question: 90\%\\ - Comment: 10\%\\ Explanation: \textless{}\textgreater{}\end{tabular}                                                                    & Unable to parse numerical scores                    \\ \bottomrule
\end{tabular}

\caption{Examples of noncompliance}
\label{tab:noncomp-examples}
\end{table*}
